Automated Focused Feedback Generation for Scientific Writing Assistance

Scientific writing is a challenging task, particularly for novice researchers who often rely on feedback from experienced peers. Recent work has primarily focused on improving surface form and style rather than manuscript content. In this paper, we propose a novel task: automated focused feedback generation for scientific writing assistance. We present SWIF$^{2}$T: a Scientific WrIting Focused Feedback Tool. It is designed to generate specific, actionable and coherent comments, which identify weaknesses in a scientific paper and/or propose revisions to it. Our approach consists of four components - planner, investigator, reviewer and controller - leveraging multiple Large Language Models (LLMs) to implement them. We compile a dataset of 300 peer reviews citing weaknesses in scientific papers and conduct human evaluation. The results demonstrate the superiority in specificity, reading comprehension, and overall helpfulness of SWIF$^{2}$T's feedback compared to other approaches. In our analysis, we also identified cases where automatically generated reviews were judged better than human ones, suggesting opportunities for integration of AI-generated feedback in scientific writing.

==> latex/bench.tex <==
\subsection{Automated Scientific Reviewing}
\paragraph{Scientific reviewing datasets and tasks}
In recent years, researchers have made significant contributions by constructing datasets of peer reviews for research purposes. These datasets typically involve the collection of papers and their corresponding reviews from prestigious conferences, laying the foundation for various labeling and annotation tasks. Aspects such as Originality, which highlight the discussion of a paper's originality in review sentences, have been instrumental in diverse studies, ranging from aspect score prediction \cite{kang} to aspect sentiment prediction \cite{chakraborty} and aspect-aware review generation \cite{yuan}. Explorations into argument and proposition types have further expanded the horizons of scientific reviewing, incorporating tasks like argument usage analysis \cite{Fromm} and proposition analysis \cite{hua} into the research landscape. Recent studies have focused on providing multi-disciplinary large-scale peer reviewing datasets, exemplified by notable works such as \citet{moprd} and \citet{nlpeer}. At the paragraph level, \citet{reviseresubmit} introduced a set of three tasks, one of which is the task of linking. This particular task focuses on establishing fine-grained relationships between sentences within the review and the corresponding paper. To facilitate this task, the authors annotated a subset of their dataset with links. Particularly relevant to our research is the work presented in \citet{aries}, which offers a real-world dataset comprising 196 human-labeled review comments aligned with their corresponding paper edits. Additionally, it contains 3.9K reviewer comments automatically matched to edits using author responses from OpenReview. This work differs from ours in that it focuses on aligning feedback to specific edits and generating revisions for scientific papers rather than generating the reviews themselves. We propose to leverage the resources mentioned above to automatically curate a dataset encompassing paragraphs from papers alongside their corresponding reviews.

\paragraph{Scientific reviewing tools} Automated scientific reviewing tools have emerged to address the challenges posed by the growing number of scientific papers. Various methods have been explored to automate or assist the peer review process, including meta-review generation \citep{wu,shen} and paper acceptance prediction \citep{deepsentipeer,checco,basuki}. Most relevant to our work are studies that focus on automatically generating reviews from the submitted paper itself. ReviewRobot \citep{reviewrobot} is an automated review generation tool that generates comments for multiple aspects, such as Originality. It operates in a pipeline process, extracting knowledge graphs (KGs) from the submitted paper, related work, and a background collection of previous papers. These KGs are used for comparisons to predict scores and extract structured evidence. Finally, generalized templates are applied to generate review sentences based on the gathered information. Another approach is ReviewAdvisor \citep{yuan}, which is inspired by state-of-the-art summarization models. It goes through two main steps: content selection, where salient text pieces are extracted from the papers, and aspect-aware summary generation based on these extracted pieces. In contrast, \citet{moprd} identified the limitations of the extract-then-generate method proposed by \citet{yuan}, particularly the loss of information. They proposed segmenting input papers based on the structure of the review comments and fine-tuning different LongFormer Encoder-Decoder \citep{led} generation models for each segment. However, the generated reviews from these methods lack the necessary specificity and tend to focus on the main aspects of the paper.To develop a valuable reviewing or writing assistant based on peer reviews, it is crucial to obtain constructive comments that can pinpoint weaknesses and propose improvements at a more granular level. Incorporating paragraph or sentence-level comments offers several advantages. Firstly, these comments are easily verifiable as they pertain to shorter sections of text, making it simpler to validate their accuracy and relevance. Additionally, aggregating these paragraph-level comments can result in an explainable final review. More recently, \cite{zachary} investigated the potential of GPT-4 in assisting the peer review process. The study involved 10 participants, each with a paper seeking feedback. Participants received evaluations from both another participant and GPT-4, and then rated the helpfulness of each feedback on a scale from 1 to 5.  The findings indicated that GPT-4 reviews garnered comparable ratings to human-generated reviews. However, the author acknowledged the stuyd's limitation in its small sample size. Furthermore, he highlighted potential avenues for future research based on his preliminary results, notably in exploring GPT-4's ability to provide reviews of a paper's low-level details - which is the aim of our study.

\subsection{Scientific Writing Assistance}
Text revision plays a crucial role in scientific writing assistance, and numerous studies have explored tools and approaches to support this process. In a recent survey by \citet{swa}, an examination of sentence revision tools used in scientific writing was presented. Acknowledging the effectiveness of commercially available tools for text revision, the study by \citet{swa} specifically focuses on three categories: sentence revision tools such as ChatGPT \footnote{\url{https://openai.com/blog/chatgpt}} and Langsmith \citep{langsmith}, grammar checkers like Grammarly \footnote{\url{https://www.grammarly.com}} and move annotators like Mover \citep{mover}. 
\paragraph{Scientific writing assistance} . While tools such as ChatGPT and Grammarly are leveraged by millions of users daily for text revision purposes, writing assistance has been thoroughly explored in the academic world. Within the realm of grammatical error correction (GEC), the study conducted by \citet{gec} provides an in-depth analysis of state-of-the-art GEC systems and approaches. For sentence revision specifically, \citet{sentrev} introduced SentRev as a novel writing assistance task that involves generating error-free, proofread versions of early draft sentences. In the context of writing analytics, move annotators \citep{movannot} were introduced to enhance students’ writing abilities and help them revise their drafts through the visualization of the structure. While these studies and tasks provide high-quality writing assistance, they focus on improving the clarity of the writing rather than providing constructive feedback on the actual research and improve the writer's publication. In our project, we specifically concentrate on the latter objective.


